Neural Particle Image Velocimetry

In the past decades, great progress has been made in the field of optical and particle-based measurement techniques for experimental analysis of fluid flows. Particle Image Velocimetry (PIV) technique is widely used to identify flow parameters from time-consecutive snapshots of particles injected into the fluid. The computation is performed as post-processing of the experimental data via proximity measure between particles in frames of reference. However, the post-processing step becomes problematic as the motility and density of the particles increases, since the data emerges in extreme rates and volumes. Moreover, existing algorithms for PIV either provide sparse estimations of the flow or require large computational time frame preventing from on-line use. The goal of this manuscript is therefore to develop an accurate on-line algorithm for estimation of the fine-grained velocity field from PIV data. As the data constitutes a pair of images, we employ computer vision methods to solve the problem. In this work, we introduce a convolutional neural network adapted to the problem, namely Volumetric Correspondence Network (VCN) which was recently proposed for the end-to-end optical flow estimation in computer vision. The network is thoroughly trained and tested on a dataset containing both synthetic and real flow data. Experimental results are analyzed and compared to that of conventional methods as well as other recently introduced methods based on neural networks. Our analysis indicates that the proposed approach provides improved efficiency also keeping accuracy on par with other state-of-the-art methods in the field. We also verify through a-posteriori tests that our newly constructed VCN schemes are reproducing well physically relevant statistics of velocity and velocity gradients.

==> diagnostics.tex <==
% \subsection{Spatial resolution test}

% This is a placeholder for a test on specific flow pattern that is reported for other NN methods.

% We perform spatial resolution test of the PIV-VCN and PIV-VCN-en models, by predicting an artificial vortex flow, given by Eq.~\ref{eq:vortex-flow}. The results are shown in Fig.~\ref{fig:vorex-flow}.
% \begin{equation}\label{eq:vortex-flow}
% \begin{array}{l}
% u(i, j)=3 \cos \left[\frac{2 \pi i}{250-0.3 i}\right] \sin \left[\frac{2 \pi j}{250-0.3 j}\right], \\
% v(i, j)=3 \sin \left[\frac{2 \pi i}{250-0.3 i}\right] \cos \left[\frac{2 \pi j}{250-0.3 j}\right]
% \end{array}
% \end{equation}

% \kolya{
% \subsection{Incompressibility test}

% This is a placeholder for incompressibility test — a request from Volodya. Not all of our datasets are incompressible.


% \subsection{Energy spectrum test}

% This is a placeholder for spectrum test — one of tests from Turbulence Diagnostics paper.


% \subsection{Velocity increments, intermittency and Q-R plane tests}

% This is a placeholder for other tests from Turbulence Diagnostics paper.
% }

% \misha{I can add description of possible tests. In fact the tests here may be richer than in my previous NN papers, as e.g. including not only velocity statistics but also scalar statistics, or even more importantnly joint statistics of the two. We can apply the tests both to actual physical velocities and also to these coming from synthetic data. Are we going to use the test in the loss function in this paper, or do we put this (most interesting part) in the path forward for now? We can state explicitly in the Sep 1 submission that we will attempt in the case of the manuscipt acceptance to incorporate diagnostics into the loss function and thus training in time for the final manuscript submission (Sep 25).}

% \kolya{Misha, treat all data as synthetic. John Hopkins data is also from CFD.}

% \misha{Kolya, I am not sure what do you mean by "treating all data as synthetic". I would like to differentiate velocity field data which is coming from CFD and data which is coming from velocity generated NOT by CFD. I call the later case synthetic.}

\subsection{Physics-Informed Diagnostics}

We apply to the Machine Learning algorithms developed in this manuscript a series of comprehensive physics-informed tests described briefly in the remainder of this Subsection. As of 09/01/20 results of the tests are not yet ready, however we expect to append them in time for submission of the final (production) version of the manuscript.

We work with the velocity fields, ${\bm v}(t;{\bm r})$, e.g. from the Johns Hopkins Turbulence Data Base \cite{JHTDB}, corresponding to one of the cases of the stationary, homogeneous, isotropic turbulence. Methodology for statistical diagnostics of ${\bm v}(t;{\bm r})$, reconstructed with Machine Learning from a single temporal snapshot (or multiple snapshots averaged over) is discussed in Appendix B of \cite{2018King}.
These basic tests include
\begin{itemize}
    \item Degree of the velocity compressibility, i.e. deviation of $(\nabla\cdot {\bm v})$ from zero (applicable to the cases where the flow we learn is incompressible). This test may also be extended to statistics of the velocity gradient tensor, $m^{\alpha\beta}\doteq \nabla^\alpha v^\beta$ (and not only to its diagonal component controlling incompressibility).
    \item Energy  Spectra, $\langle |{\bm v}_k|^2\rangle$, where  ${\bm v}_k$ is the spatial Fourier transform of ${\bm v}(t,{\bm r})$, over the range of  scales and respective $k$-harmonics. ($\langle\cdots\rangle$ stands for spatial, over snapshot, and temporal, over many snapshots, averaging.)
    \item Intermittency test of scaling of the velocity increments, $\langle |{\bm v}(t,{\bm r}_0+{\bm r})-{\bm v}(t,{\bm r}_0+{\bm r})|^n$, studied as functions of the order $n$ and of the scale $r$, scanning through the inertial range of turbulence (ranging from the smallest, viscous scale all the way to the largest, energy containing scale of turbulence).
    \item Statistics of the velocity gradient tensor, $m^{\alpha\beta}$, coarse-grained over a scale $r$ from the inertial range of turbulence (i.e. spatially convoluted with a kernel, typically of Gaussian shape, of size $r$). Specifically,  we usually aim to reconstruct statistics of the second, $Q$, and third, $R$, invariants of the coarse-grained velocity tensor.  
\end{itemize}
These tests of velocity statistics can also be extended to statistics of the density field, $\rho(t,{\bm r})$:
\begin{itemize}
    \item Density spectra, $\langle |\rho_k|^2\rangle$, where $\rho_k$ is the spatial Fourier transform of $\rho(t,{\bm r})$, over the range of scales and respective $k$-harmonics.
    \item Intermittency of density (typically much stronger pronounced than intermittency of velocity) testing scaling of the density increments, $\langle |\rho(t,{\bm r}'+{\bm r})-\rho(t,{\bm r}')|^n\rangle$, as functions of $n$ and $r$, where $r$ scans scales from the inertial range of turbulence.
    \item Statistics of the density gradient vector, $\nabla\rho$, with a special focus on the tails of the probability distribution. 
\end{itemize}
It is also of interest to test mixed objects such as
\begin{itemize}
    \item mean flux of density fluctuations, $\langle \rho(t,{\bm r}'+{\bm r}) v^\alpha(t,{\bm r}')\nabla^\alpha \rho(t,{\bm r}')\rangle$, as a function of $r$, and respective higher order moments (statistics/intermittency) of the flux. 
\end{itemize}

Notice that the diagnostic is focused on evaluating simultaneous (the same time) statistics of velocity and density. Even richer tests can be designed to analyse temporal, i.e. different time, correlations in Eulerian (not moving with the flow) and Lagrangian (evolving with the flow) frames. 

The extended diagnostics of turbulence is expected to be useful not only to a-posteriori test of the Machine Learning schemes but also for imposing a-priori physics-informed guidance.  In particular, we envision incorporating physics-informed regularizations to the loss function aimed at minimizing deviations of the statistical characteristics which show the largest mismatch in the a-posteriori tests.


%\misha{Kolya,  I stop here. There are a number of additional objects we can add, noticeably these discussing different time correlations in Eulerian  (easy but less interesting) and Lagrangian (more interesting but also more challenging) frames. (All tests suggested above are "simultaneous", i.e. testing correlations within a single snapshot and not cross-correlations between different snapshots.) However, I feel that these tests of different times (snapshots), as well as planting some mix of the tests into the loss function, should be moved to discussion of the "path forward".}

